The effect of obstacles near a silo outlet on the discharge of soft spheres

Soft smooth particles in silo discharge show peculiar characteristics, including, for example, non-permanent clogging and intermittent flow. This paper describes a study of soft, low-frictional hydro\-gel spheres in a quasi-2D silo. We enforce a more competitive behavior of these spheres during their discharge by placing an obstacle in front of the outlet of the silo. High-speed optical imaging is used to capture the process of discharge. All particles in the field of view are identified and tracked by means of machine learning software using a MASK R-CNN algorithm. With particle tracking velocimetry (PTV), the fields of velocity, egress time, packing fraction, and kinetic stress are analysed in this study. While in pedestrian dynamics, the placement of an obstacle in front of a narrow gate may reduce the stress near the exit and enable a more efficient egress, the effect is opposite for our soft grains. Placing an obstacle above the orifice always led to a reduction of the flow rates, in some cases even to increased clogging probabilities.

==> flowchart.tex <==

% Drawing part, node distance is 1.5 cm and every node
% is prefilled with white background
\begin{adjustbox}{max width=\textwidth}
\begin{tikzpicture}[node distance=1.5cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \node (start)             [activityStarts]              {list of particle information};
  \node (onCreateBlock)     [process, below of=start]          {condition for stagnant zone};
  \node (onStartBlock)      [activityStarts, below of=onCreateBlock]   {list of moving particles};
  \node (onResumeBlock)     [process, below of=onStartBlock]   {condition for particles flowing out};
  \node (activityRuns)      [activityRuns, below of=onResumeBlock]
                            {list of particles not out yet};
  \node (onPauseBlock)      [process, below of=activityRuns]
                            {search ending points close to positions of those particles flowing out};
  \node (onDecideBlock)     [process, below of=onPauseBlock] 
                            {particles got found};
  \node (onStopBlock)       [process, below of=onDecideBlock]
                            {update duration $\Delta t + \overline{\Delta t ^\prime}$};
  \node (onDestroyBlock)    [process, below of=onStopBlock] 
                            {concatenate 2 lists};
%  \node (onPauseBlock)      [process, below of=activityRuns, yshift=-1cm]
%                                                                {search ending points close to positions of those particles flowing out};
%  \node (onStopBlock)       [process, below of=onPauseBlock, yshift=-1cm]
%                           {update duration $\Delta t + \overline{\Delta t ^\prime}$};
%  \node (onDestroyBlock)    [process, below of=onStopBlock, yshift=-1cm] 
%                                                              {concatenate 2 lists};
  \node (onRestartBlock)    [process, right of=onResumeBlock, xshift=5cm]
                            {list of particles flowing out};
  \node (ActivityEnds)      [startstop, left of=onCreateBlock, xshift=-5cm]
                            {list of stationary particles};
  \node (ActivityDestroyed) [startstop, below of=onDestroyBlock]
                            {list of particle information updated};     
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
  \draw[->]             (start) -- (onCreateBlock);
  \draw[->]     (onCreateBlock) -- node[xshift=0.5cm,text width=0.5cm]{NO}(onStartBlock);
  \draw[->]     (onCreateBlock) -- node[yshift=0.5cm,text width=0.6cm]{YES}(ActivityEnds);
  \draw[->]      (onStartBlock) -- (onResumeBlock);
  \draw[->]     (onResumeBlock) -- node[xshift=0.5cm,text width=0.5cm]{NO}(activityRuns);
  \draw[->]     (activityRuns)  -- (onPauseBlock);
  \draw[->]     (onPauseBlock)  -- (onDecideBlock);
  \draw[->]     (onDecideBlock)  -- (onStopBlock);
  \draw[->]    (onResumeBlock) -- node[yshift=0.5cm,text width=0.6cm]{YES}(onRestartBlock);
  \draw[->]    (onDestroyBlock) -- (ActivityDestroyed);
  \draw[->]    (onStopBlock.east) -| node[yshift=1.5cm,text width=3cm]
               {add updated particle} (onRestartBlock);
  \draw[->]    (onDecideBlock.west) --++(-6,0) --++ (0,3) -- node[xshift=-2.5cm, yshift=-2.4cm,text width=4cm]{expand searching range}(activityRuns.west);
  \draw[->]   (onRestartBlock.east) --++ (0.5,0) --++ (0,-7.5) -- (onDestroyBlock.east);
  \draw[->]   (ActivityEnds.west) --++ (-0.5,0) --++ (0,-10.5) -- (onDestroyBlock.west);
%  \draw[->]      (activityRuns) -- node[text width=4cm]
%                                   {Another activity comes in
%                                    front of the activity} (onPauseBlock);
%  \draw[->]      (onPauseBlock) -- node {The activity is no longer visible}
%                                   (onStopBlock);
%  \draw[->]       (onStopBlock) -- node {The activity is shut down by
%                                   user or system} (onDestroyBlock);
%  \draw[->]       (onStopBlock) -| node[yshift=1.25cm, text width=3cm]
%                                   {The activity comes to the foreground}
%                                   (onRestartBlock);
%  \draw[->]      (onPauseBlock) -| node(priorityXMemory)
%                                   {higher priority $\rightarrow$ more memory}
%                                   (ActivityEnds);
%  \draw           (onStopBlock) -| (priorityXMemory);
%  \draw[->]     (ActivityEnds)  |- node [yshift=-2cm, text width=3.1cm]
%                                    {User navigates back to the activity}
%                                    (onCreateBlock);
%  \draw[->] (onPauseBlock.east) -- ++(2.6,0) -- ++(0,2) -- ++(0,2) --                
%     node[xshift=1.2cm,yshift=-1.5cm, text width=2.5cm]
%     {The activity comes to the foreground}(onResumeBlock.east);
\end{tikzpicture}
\end{adjustbox}
